MagicDec: Breaking the Latency-Throughput Tradeoff for Long Context Generation with Speculative Decoding

Large Language Models (LLMs) have become more prevalent in long-context applications such as interactive chatbots, document analysis, and agent workflows, but it is challenging to serve long-context requests with low latency and high throughput. Speculative decoding (SD) is a widely used technique to reduce latency losslessly, but the conventional wisdom suggests that its efficacy is limited to small batch sizes. In MagicDec, we show that surprisingly SD can achieve speedup even for a high throughput inference regime for moderate to long sequences. More interestingly, an intelligent drafting strategy can achieve better speedup with increasing batch size based on our rigorous analysis. MagicDec first identifies the bottleneck shifts with increasing batch size and sequence length, and uses these insights to deploy SD more effectively for high throughput inference. We leverage draft model with sparse KV cache to address the KV bottleneck, which scales with both sequence length and batch size. Additionally, we propose a theoretical model to select the optimal drafting strategy for maximum speedup. Our work highlights the broad applicability of speculative decoding in long-context serving, as it can enhance throughput and reduce latency without compromising accuracy. For moderate to long sequences, we demonstrate up to 2.51x speedup for Llama3.1-8B when serving batch sizes ranging from 32 to 256 on various types of hardware and tasks.

==> Sections/intro_ranajoy.tex <==
\section{Introduction}

The emergence of extremely long-context models \citep{llama3.1, qwen2.5, liu2023visualinstructiontuning} has led to the growing popularity of many long-context applications such as Retrieval Augmented Generation \citep{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp}, code generation \citep{copilot, codewhisperer, chen2021evaluatinglargelanguagemodels}, document summarization, to name a few. From a commercial perspective, it is crucial to deliver these long-context applications with minimal latency and maximum throughput. While low latency is essential for maintaining a positive user experience in interactive applications like chatbots \citep{achiam2023gpt, claude3, gemini1.5, bingchat}, high throughput helps reduce serving costs. However, current Large Language Model (LLM) serving systems face a trade-off between latency and throughput while handling long-context requests.

The decoding phase of a single request is primarily constrained by parameter loading cost, making batching an effective strategy to improve throughput. However, when dealing with long contexts and large batch sizes, this approach introduces a substantial increase in Time-Between-Tokens (TBT). This increased is caused by the introduction of two new bottlenecks that scale with either batch-size or sequence length - computation cost and KV cache loading. As a result, existing serving systems are forced to prioritize either throughput or latency, inevitably sacrificing the other metric. For example, throughput-optimized serving pipelines like vLLM \cite{vllm}, ORCA \cite{yu2022orca} suffer from high token-wise latency, while latency-improving methods like Speculative Decoding \citep{leviathan2022fast, xia2023speculativedecodingexploitingspeculative, chen2023accelerating} are often worse than autoregressive decoding for high-throughput serving \cite{liu2024optimizingspeculativedecodingserving, su2023synergyspeculativedecodingbatching}. Although compression methods such as quantization \citep{frantar2023gptqaccurateposttrainingquantization,xiao2024smoothquantaccurateefficientposttraining,hooper2024kvquant10millioncontext} and pruning \citep{ma2023llmprunerstructuralpruninglarge, sun2024simpleeffectivepruningapproach} can improve both throughput and latency, they often come at the cost of reduced generation quality. So, we pose the following question:
\begin{quote}
\itshape Can we simultaneously improve \textbf{throughput} and \textbf{latency} without sacrificing \textbf{accuracy}, particularly for long sequences?
\end{quote}

To answer this question, we revisit the efficacies of Speculative Decoding (SD). While its throughput performance has been well-studied in short sequence length regime (input length=output length=128) \cite{liu2024optimizingspeculativedecodingserving, su2023synergyspeculativedecodingbatching}, a thorough analysis in the long-context and large batch-size regime is still due. According to the recent studies, the batch inference performance of SD has been restricted primarily due to two challenges. First, for larger batches, the linear layers fully utilize the compute resources that SD otherwise uses for efficient verification in a more memory-bound scenario. Second, in a large-batch regime, the draft token acceptance rate is of the essence because otherwise the expensive verification process has to be performed for too many incorrectly speculated tokens. Unfortunately, it is often difficult to find suitable small draft models that can achieve a reasonable acceptance rate. [TODO: For instance, get acceptance rate for short sequence from RULER, can not find from goodput paper]. 

\begin{figure}[t]
    \begin{center}
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/kv_sup/memory_vs_acc.pdf}
            \subcaption{}\label{fig:kv-acc-rates}
        \end{minipage}
        \hfill
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/throughput-latency/TinyLlama-1.1B-intermediate-step-1431k-3T_consolidated_max_throughput_vs_latency_prefill_8000.pdf}
            \subcaption{}\label{fig:throughput-latency-a}
        \end{minipage}
        \hfill
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/throughput-latency/TinyLlama-1.1B-intermediate-step-1431k-3T_preliminary_throughput_ratio_all_prefills.pdf}
            \subcaption{}\label{fig:throughput-latency-b}
        \end{minipage}
        \caption{\small{(a) Comparison of acceptance rates between small draft model ( model suite) with full KV cache and self-speculation with sparse KV cache for target model \qwenlarge. The acceptance rates and memory footprint ratios are computed for context-length of 100,000 and batch-size of 64 on PG-19 dataset. (b) Throughput of autoregressive and SD against per-token latency for context-length of 8k with target model \llamalong  and draft model \tinyllama}.
        (c) Throughput ratio of SD to autoregressive across latency budgets, showing that SD improves throughput for sequences longer than 1024 target model \llamalong  and draft model \tinyllama.}
        \label{fig:throughput-latency}
    \end{center}
\end{figure}

However, our in-depth analysis of LLM inference reveals that the first challenge is limited to short sequence lengths only. Similarly, the second challenge can be overcome by better drafting strategies. Our hypothesis is based on the following key insights.

\underline{\textit{KV cache is the new primary bottleneck}}: 
In the long-context and large batch size regime, the KV cache outgrows the model parameter memory footprint and continues to increase with batch size. Moreover, because of the high peak-flops to memory-bandwidth ratio of modern GPUs, the KV loading time increases much more than the computation time for larger batches, making LLM more memory-bound (see Fig. \ref{fig:kv-bottleneck}). Because SD uses the KV budget for both decoding and verification, the extra computation cost of the latter does not affect the verification to decoding cost ratio much. 

\underline {\textit{Speculation is easier with compressed KV than with lightweight draft models}}:
We observe that in the large batch-size and long-context regime, a KV sparsification-based drafting scheme can solve the low acceptance rate problem of small draft models. Fig. \ref{fig:kv-acc-rates} demonstrates that self-speculation with \qwenlarge achieves better acceptance rates than smaller models in the \wrapttt{Qwen2.5} \citep{qwen2.5} model suite when working with the same memory constraints.  

Building upon these insights, we propose MagicDec that exploits the high acceptance rates of sparse KV cache-based draft models and provides better latency-throughput trade-off in a long-context and large batch-size regime. More interestingly, our proposed method can achieve \textbf{better speed-up with increasing batch-size}, contrary to the prior belief about SD's ineffectiveness for larger batches.

\begin{itemize}
    \item In Section \ref{subsec:bottleneck-shift}, we analyze the bottleneck shift in LLM inference with increasing batch-size and sequence length to show why SD can be beneficial even for larger batches. We theoretically show that beyond a sequence length that is specific to the hardware and model pair, verification to target decoding cost ratio does not increase much with batch-size.
    \item In Section \ref{subsec:sparse_kv} and Section \ref{subsec:better-acc-rate}, we illustrate why sparse KV cache is an essential drafting strategy in our regime of interest.
    \item In Section \ref{subsec:ablation}, we conduct an ablation study examining various KV sparsification techniques, including StreamingLLM \citep{xiao2024efficientstreaminglanguagemodels}, SnapKV \citep{li2024snapkvllmknowslooking}, topk-attention \citep{gupta2021memoryefficienttransformerstopkattention}. Our goal is to identify an optimal balance between draft generation cost and acceptance rate. Furthermore, we provide a theoretical analysis demonstrating the effectiveness of a tree-based speculation method, that leverages the enhanced acceptance rate.
\end{itemize}

==> Sections/introduction.tex <==
\section{Introduction}

[\textcolor{red}{Problem and why is it interesting}]\\
The landscape of language models has changed dramatically, with models capable of processing extremely long context lengths becoming increasingly prevalent \citep{llama3.1, qwen2.5, liu2023visualinstructiontuning}. In addition, the growing popularity of long-context applications such as Retrieval Augmented Generation \cite{lewis2021retrievalaugmentedgenerationknowledgeintensivenlp} has sparked significant interest in serving large batches of long-context requests more efficiently. Optimizing latency and throughput are both important because low latency serves application requirements such as user experience in interactive chatbots 
 \citep{achiam2023gpt, gemini1.5, claude3}. On the other hand, high throughput reduces serving costs \citep{narayan2022foundationmodelswrangledata, chen2021spreadsheetcoderformulapredictionsemistructured}. 
However, it has been challenging to achieve both high throughput and low latency for LLM serving. The autoregressive token generation during the LLM decode phase makes it highly memory-bound, leading to low throughput. Batching can significantly help to utilize GPU resources and improve throughput, but typically it will increase the TBT (time-between-tokens)\citep{agrawal2024tamingthroughputlatencytradeoffllm}. 

% In this paper, we analyze this bottleneck shift to improve throughput-latency trade-off particularly for long-context serving. 

[\textcolor{red}{Why existing solutions failed}]\\
Autoregressive decoding is inherently a memory-bound process. Hence, batching \citep{vllm, yu2022orca,agrawal2024tamingthroughputlatencytradeoffllm} has been the most effective approach to improve throughput, as it allows us to share the parameter loading cost across large batches. However, in our regime of interest, batching becomes ineffective, as it results in a substantial increase in latency. With increasing batch size, the linear layers in LLMs start to become compute-bound after which any increase in batch size will significantly increase computation latency. Moreover, for moderate to long sequences, a new memory bottleneck emerges that can not be hidden by batching - the \textit{KV cache bottleneck}. Consequently, improving throughput for long-context requests has been a non-trivial problem that can not be solved by batching alone. 

% Unlike parameter loading, this new memory bottleneck scales with batch-size making batching ineffective in our regime of interest.
% Although  lossy methods like quantization \citep{frantar2023gptqaccurateposttrainingquantization,xiao2024smoothquantaccurateefficientposttraining,hooper2024kvquant10millioncontext} and pruning \citep{ma2023llmprunerstructuralpruninglarge, sun2024simpleeffectivepruningapproach} can improve both latency and throughput but often compromise generation quality. 

On the other hand, Speculative Decoding (SD) \citep{leviathan2022fast, xia2023speculativedecodingexploitingspeculative, chen2023accelerating} improves latency at the cost of increased computation, which can become prohibitive for large batches. In this method, a lightweight draft model is used to efficiently generate multiple tokens that are verified in parallel by the target model. In the low batch-size setting, this is effective because compute resources are under-utilized due to the dominant parameter loading cost. However, as batch-size increases, verification becomes significantly more expensive than decoding. This is exacerbated by a low draft token acceptance rate, because the target LLM wastes a lot of time in verifying incorrectly speculated tokens. As a result, speculative decoding is avoided in the large batch size regime \citep{liu2024optimizingspeculativedecodingserving,su2023synergyspeculativedecodingbatching,miao2023specinfer}.

\begin{figure}[t]
    \begin{center}
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/kv_sup/memory_vs_acc.pdf}
            \subcaption{}\label{fig:kv-acc-rates}
        \end{minipage}
        \hfill
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/throughput-latency/TinyLlama-1.1B-intermediate-step-1431k-3T_consolidated_max_throughput_vs_latency_prefill_8000.pdf}
            \subcaption{}\label{fig:throughput-latency-a}
        \end{minipage}
        \hfill
        \begin{minipage}{0.32\textwidth}
            \includegraphics[width=\textwidth]{Plots/throughput-latency/TinyLlama-1.1B-intermediate-step-1431k-3T_preliminary_throughput_ratio_all_prefills.pdf}
            \subcaption{}\label{fig:throughput-latency-b}
        \end{minipage}
        \caption{\small{(a) Comparison of acceptance rates between small draft model ( model suite) with full KV cache and self-speculation with sparse KV cache for target model \qwenlarge. The acceptance rates and memory footprint ratios are computed for context-length of 100,000 and batch-size of 64 on PG-19 dataset. (b) Throughput of autoregressive and SD against per-token latency for context-length of 8k with target model \llamalong  and draft model \tinyllama}.
        (c) Throughput ratio of SD to autoregressive across latency budgets, showing that SD improves throughput for sequences longer than 1024 target model \llamalong  and draft model \tinyllama.}
        \label{fig:throughput-latency}
    \end{center}
\end{figure}

% Throughput vs. Latency for \tinyllama\ speculating \llamalong\ at different prefill lengths. \textbf{(b)} Throughput of autoregressive and SD against per-token latency for prefill 8000. \textbf{(c)} Throughput ratio of SD to autoregressive across latency budgets, showing that SD improves throughput for sequences longer than 1024.

[\textcolor{red}{Key Challenges and Insights to overcome them}]\\
However, despite the recent surge of interest in the long-context and high batch-size regime, the study of SD has been limited to large batches of small sequences only \citep{liu2024optimizingspeculativedecodingserving,su2023synergyspeculativedecodingbatching}. In this work, we examine speculative decoding in this particular regime and pose the following question:
\begin{quote}
    \itshape Can we use Speculative Decoding to simultaneously improve throughput and latency, particularly for long sequences?
\end{quote}

In Sec. \S \ref{sec:factors}, we show that for moderate to long sequences, the verification to decoding cost ratio does not grow too much with increasing batch size. Hence, an effective drafting strategy can in fact make SD useful even for large batches. 

However, there are some key challenges that prevents us from utilizing SD in the traditional way. First, small draft models are often unable to scale well with increasing batch-size. As illustrated in Fig. \ref{fig:7bkv} and Fig. \ref{fig:8bkv}, the KV memory footprint of the draft model can be so substantial that it can outweigh the benefits of saving parameters. Second, the acceptance rates of lightweight draft models are often too low to be useful in a large batch-size regime. A low draft token acceptance rate penalizes the verification cost more in this setting. Third, suitable small draft models are not always readily available for certain models such as \llamathree because of mismatched vocabulary size. We overcome these challenges on the basis of the following key insights.

\underline{\textit{KV cache is the new primary bottleneck}}: 
In the long-context and large batch size regime, the KV cache outgrows the model parameter memory footprint and continues to increase with batch size. Moreover, because of high peak-flops to memory-bandwidth ratio of modern GPUs, the KV loading time increases much more than the computation time for larger batches (see Fig. \ref{fig:kv-bottleneck}). This phenomenon allows the verification to be reasonably close to the target decoding cost. In addition, it highlights the importance of optimizing the KV loading cost while designing a drafting strategy.

\underline {\textit{Speculation is easier with compressed KV than with lightweight draft models}}: 
We empirically show that at the same compression level, KV sparsification is much more effective than model parameter reduction with smaller draft models. For instance, Fig \ref{fig:kv-acc-rates} shows that for the target model \qwenlarge, self-speculation achieves a much better acceptance rate compared to smaller draft models in the same model suite with full KV cache.

% we device drafting strategies based on sparse KV cache. This particular drafting strategy not only helps SD to achieve better throughput, but also enables it to achieve even \textbf{better speed-up for larger batches}. As Figure \ref{fig:throughput-latency} illustrates, for a given latency budget, SD has higher throughput than autoregressive decoding, and the efficacy of SD is evidently greater for longer sequences. Moreover, if we can allow a higher latency budget, we can improve throughput even more with MagicDec.

[\textcolor{red}{Our contribution}]\\
Building upon these insights, we propose KV sparsification as a necessary drafting strategy while serving large batches of long requests. Unlike traditional SD, the draft to target cost ratio decreases with increasing batch-size, (discussed in detail in Sec. \S \ref{sec:factors}), helping SD accelerate batch inference. More interestingly, the superior acceptance rate (~90 - 92\%) and the decreasing draft-to-target cost ratio allow us to \textit{speculate more tokens in a higher batch-size regime}, resulting in \textit{\textbf{better speed-up for larger batches}}.\\
The main contributions of our work are:
\begin{enumerate}
    \item We perform theoretical analysis of LLM inference to better understand the efficacy of speculative decoding in large batch-size, long context regime.
    \item We identify KV sparsification as an essential drafting strategy that allows SD to improve both latency and throughput in our regime of interest.
    \item We perform a thorough ablation study across different KV sparsification methods such as StreamingLLM \cite{xiao2024efficientstreaminglanguagemodels}, SnapKV \cite{li2024snapkvllmknowslooking}, top-k attention \cite{gupta2021memoryefficienttransformerstopkattention}, etc. to strike a better balance between the draft cost and the acceptance rate.
\end{enumerate}
% Unlike traditional SD, self-speculation with sparse KV cache is not limited by vocabulary mismatch issue. Furthermore, KV sparsification improves the acceptance rate, which is maintained even for large batch sizes. In addition, our proposed approach provides the flexibility to decide sparsification level to strike the best balance between draft cost and acceptance rate. 

% However, there are different strategies to compress KV cache. To choose between different KV compression strategies, we perform a thorough ablation study to strike the right trade-off between KV compression overhead and acceptance rate. Furthermore, we present tree-based speculation strategies that can drastically improve token acceptance rates with minimal increase in verification time.

% The main contributions of our work are:
% \begin{enumerate}
%     \item We perform theoretical analysis of LLM inference performance to identify suitable drafting strategies for SD in large batch-size and long-context regime. We challenge the existing belief that SD is ineffective in improving throughput. On the contrary, we exhibit even better speed-up for larger batches when the context length is beyond a certain threshold.
%     \item We propose KV sparsification as an essential drafting strategy in the large batch-size, long-context regime based on our theoretical analysis.
%     \item We perform extensive ablation studies on various KV sparsification techniques. Additionally, we propose a tree-based speculation approach to achieve even better speed-ups.
% \end{enumerate}

[\textcolor{red}{How do you evaluate}]\\
TODO: Add speed-up after final testing

==> Sections/observations.tex <==
\section{Observations}
\subsection{Shift in bottleneck with increasing batch-size}
\label{subsec:bottleneck-shift}
In this section, we discuss how the LLM operation bottleneck shifts as the batch-size increases for long-context sequences and its implications on the efficacies of SD. 
When sequence length is too short, SD has a detrimental effect on batch inference efficiency \cite{liu2024optimizingspeculativedecodingserving, su2023synergyspeculativedecodingbatching}. Because with increasing batch-size, the arithmetic intensity of the linear layers improve, pushing these layers to the compute-bound regime. Consequently, the underutilized compute resources SD uses for an efficient verification process begins to deplete. 

However, for moderate to long sequences, increasing batch-size makes the model inference more memory-bound instead due to the introduction of a new memory bottleneck - the KV cache. This new memory bottleneck allows the verification cost to remain reasonably close to the target decoding time. Because verification and decoding share the same KV budget, their KV cache loading costs are equivalent. In addition, due to the high peak-flops / memory-bandwidth ratio of the modern GPUs, the increase in KV loading time with batch-size is more substantial compared to that of the computation time (see Fig. \ref{fig:kv-bottleneck}). Consequently, even though the compute-bound linear layers increase the verification cost, its effect is diminished by the KV bottleneck. 

Fig. \ref{fig:theoretical-arithmetic-intensity} illustrates that for every model and hardware pair, there exists a critical sequence length, beyond which the LLM batch inference becomes more memory-bound. Hence, SD is expected to improve batch latency beyond this critical sequence length.

\subsection{Importance of Sparse KV Cache}
\label{subsec:sparse_kv}

\begin{figure}[t]
    \centering
    \begin{minipage}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/Theoretical/time_breakdown-llama31-8b.pdf}
        \subcaption{\llamathree}
         \label{fig:kv-bottleneck}
    \end{minipage}
    \hfill
    \begin{minipage}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/Theoretical/mem_ratios/draft_to_target_memory_llama3_8b_vs_70b.pdf}
         \subcaption{\llamathree/\llamathreelarge}
         \label{fig:8bkv}
        %\label{fig:theoretical-speedup-seqlen}
    \end{minipage}
    \hfill
    \begin{minipage}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/Theoretical/mem_ratios/draft_to_target_memory_llama2_7b_vs_70b.pdf}
        \subcaption{\llamatwo/\llamatwolarge}
        \label{fig:7bkv}
        % \label{fig:theoretical-arithmetic-intensity}
    \end{minipage}
    \caption{\small{Theoretical analysis of KV cache bottleneck in speculative decoding.} \textbf{(a)} Time breakdown of \llamathree vs batch size (input length=16384, hardware=8xH100s): KV cache, weights, activations loading, and compute. \textbf{(b,c)} Draft/target memory ratio vs batch size across different sequence lengths for \llamathree/\llamathreelarge and \llamatwo/\llamatwolarge architectures. }
    
\end{figure}

Traditionally SD utilizes a light-weight draft model to address the parameter loading bottleneck during autoregressive decoding. However, in the regime of large batch-size and long sequence length, we find KV compression is a better drafting strategy than opting for smaller models. 

This observation is supported by how the LLM bottleneck shifts with increasing sequence length and batch size. Fig. \ref{fig:kv-bottleneck} illustrates how the KV bottleneck of \llamatwo model starts to dominate over the workloads like parameter loading and computation for a moderately long context length of 4096. This is because unlike model parameters, the KV cache grows linearly with batch-size, drawing more attention in the high throughput regime. In the cases of \llamathree for \llamathreelarge and \llamatwo for \llamatwolarge, the draft models can occupy up to $38\sim140\%$ memory footprint of target models (\Cref{fig:7bkv,fig:8bkv})due to the fact that 
 $\mathrm{dim}_{kv}/\mathrm{dim}_{model}$ is higher. Hence, in our regime of interest, small draft models are not sufficient and sparse KV-based drafting is quite beneficial\citep{sun2024triforcelosslessaccelerationlong}. 
This can be seen in Figure \ref{fig:theoretical-draft-verificaiton}, which illustrates how ${T_D}/{T_T}$ for self-speculation approaches 0 with increasing sequence length for batch size 256. 

Additionally, a sparse KV-based drafting strategy offers the flexibility of choosing the required sparsity level to strike a balance between the acceptance rate and draft efficiency. Moreover, a mismatch in vocabulary size often makes it difficult to find a suitable small draft model for target models such as \llamathree. In such cases, sparse KV-based self-speculation could be the only available drafting option.  

\subsection{Sparse KV gives higher acceptance rates than small draft}
\label{subsec:better-acc-rate}

In addition to the superior memory saving capabilities, KV cache sparsification proves to be a more cost-effective way of enhancing token acceptance rate, especially in a long-context, high batch-size regime. At a higher level of compression factor,  KV sparsification can achieve a better acceptance rate than smaller draft models. We illustrate this phenomenon for the \wrapttt{Qwen} \cite{qwen2.5} model suite. When using a context length of 100,000 tokens and a batch size of 64, we found that self-speculation provides a better balance between acceptance rate and memory savings compared to using small draft models for speculating on the \qwenlarge target model.

TODO: Adding plot for \llamathreelarge self-spec vs \llamathree expected speedups with increasing batch-size. The former should have increasing speed-up. The latter will have diminishing speed-ups.
% As discussed in Sec. \S \ref{sec:factors}, at the same KV sparsification level, the draft to target cost ratio decreases with increasing batch size. On the other hand, the efficacy of a small draft model is reduced.



==> Sections/points.tex <==
\subsection{Problem To Solve}
\begin{enumerate}
    \item High-throughput serving of long context requests
    \item Loss-less method with better latency-throughput trade-off
    % \item Recommending a system-design choice for large-scale distributed serving system - move it to future works  
\end{enumerate}

\subsection{Why is it interesting?}
\begin{enumerate}
    \item Low latency and high throughput both are important. Low latency for interactive use cases. High-throughput serving helps generate more revenue for the industries. 
    \item With the advent of long-context models, serving large batches of long contexts has become ubiquitous. For example, RAG-based pipelines often have to serve large batches of queries concatenated with retrieved long documents.
\end{enumerate}


\subsection{Why is it a hard problem?}
\begin{enumerate}
    \item Latency-throughput trade-off. Batching is the most useful way of increasing throughput. But increasing batch size often increases latency. Especially in very high batch-size regime, where parameter loading time is not the primary bottleneck anymore, both computation time and KV cache loading time increase with batch size, resulting in high latency.
    % \item Quantization and pruning methods can improve latency and throughput, but at the expense of generation quality.
    \item Speculative decoding can maintain quality. But when used in the usual way, it does not work well in large batch-size regime because of low acceptance rate, increased draft time and verification time.
    \item low acceptance rate problem (small draft model)
    \item low token utilization creates problem in compute-bound regime.
\end{enumerate}

\subsection{What is your insight? Why you can solve the problem? what is your approach principle?}
\begin{enumerate}
    \item In large batch-size and sequence length regime, the bottleneck shifts towards KV loading. So, with increasing batch-size, verification of speculated tokens does not become prohibitively large compared to target decoding time.
    \item Because KV loading is the new bottleneck, there is an opportunity to design better draft models by compressing KV memory. 
    \item We notice that KV compression is much easier than model compression as far as acceptance rate is concerned. So, we focus on algorithms to compress KV effectively.
    % \item Dynamic KV compression increases draft cost. Static KV selection is efficient, but is expected to be less accurate. However, we notice that a static KV selection scheme can often cover a large portion of dynamically selected items. Thus, it provides a better efficiency-accuracy trade-off. - move it to contribution
\end{enumerate}


\subsection{How do you convince the audience? How do you evaluate it?}
\begin{enumerate}
    \item Why studying decoding only? 
    % Disaggregated serving helps us decouple prefill and decoding stages. So we can focus on decoding separately - move to future works
    \item For speedup with batch size:
    \begin{enumerate}
        \item Theoretical verification/decoding cost ratios vs batch size. 
        \item Theoretical draft/target cost ratios vs batch size.
        \item empirical speed-ups.
    \end{enumerate}
    \item Draft selection:
    \begin{enumerate}
        \item small model acceptance rate vs small KV acceptance rate (70B vs 8B model performance?)
        \item adjustable KV size ratio - move to methodology 
        \item static vs dynamic KV selection: top-k overlap ratio among next generated tokens. - ablation studies for different tasks
    \end{enumerate}
        
\end{enumerate}

==> Sections/related-works.tex <==
\section{Related Works}
\label{sec:related-work}

Numerous efforts have been made to improve the latency and throughput of LLMs. Although methods like Flash decoding \citep{dao2023flashattention2fasterattentionbetter}, Flash decoding++\citep{hong2023flashdecoding++}, FasterTransformers\citep{fastertransformer} have performed system optimizations to improve latency, speculative decoding\citep{leviathan2022fast, xia2023speculativedecodingexploitingspeculative, chen2023accelerating} has emerged as a novel sampling algorithm to speed up inference. On the other hand, batching has been a natural technique to improve GPU utilization and throughput. To make batching more effective, continuous batching \citep{vllm, yu2022orca, prabhu2024vattentiondynamicmemorymanagement} and chunked prefill \citep{agrawal2024tamingthroughputlatencytradeoffllm} techniques have proposed intelligent batch scheduling techniques. Although these techniques can address the problems arising from heterogeneous batches with unequal context and generation lengths, they cannot solve the memory-bound problem of autoregressive decoding. In our work, we have considered the orthogonal direction of homogeneous batches, and therefore the aforementioned methods are complementary to our observation.  

In our work, we have used speculative decoding as a method to balance the throughput-latency trade-off. We have particularly focused on draft models with sparse KV cache. This approach is motivated by the recent finding in Triforce \cite{sun2024triforcelosslessaccelerationlong} that self-speculation with sparse KV is an effective draft choice when KV loading is the main bottleneck. While Triforce is designed for small batches of extremely long sequences, we have focused on large batches of moderate to long sequences in our work.  

Although promising for single batch requests, Speculative Decoding poses new challenges when implemented with batch support. Because the number of accepted tokens in SD follows a truncated geometric distribution \cite{leviathan2022fast}, the average accepted length can vary throughout the batch, leading to misalignment of the sequence lengths. \citep{qian2024bassbatchedattentionoptimizedspeculative} have optimized the attention kernels to take care of this unequal number of accepted tokens across the batch. However, as previously reported, the excess computation for SD could be restrictive in a large batch size regime \citep{liu2024optimizingspeculativedecodingserving, su2023synergyspeculativedecodingbatching, miao2023specinfer, sun2024triforcelosslessaccelerationlong}. Hence, \citep{liu2024optimizingspeculativedecodingserving,su2023synergyspeculativedecodingbatching} suggest a reduction in speculation length with increasing batch size.

These findings imply that SD is not as effective in improving throughput; however, we notice that these observations are limited to a very small sequence-length regime. In our work, we focus on the relatively longer sequences that have been ubiquitous in practice. 
